Distributed Evaluation of Subgraph Queries Using Worstcase Optimal LowMemory Dataflows

We study the problem of finding and monitoring fixed-size subgraphs in a continually changing large-scale graph. We present the first approach that (i) performs worst-case optimal computation and communication, (ii) maintains a total memory footprint linear in the number of input edges, and (iii) scales down per-worker computation, communication, and memory requirements linearly as the number of workers increases, even on adversarially skewed inputs. Our approach is based on worst-case optimal join algorithms, recast as a data-parallel dataflow computation. We describe the general algorithm and modifications that make it robust to skewed data, prove theoretical bounds on its resource requirements in the massively parallel computing model, and implement and evaluate it on graphs containing as many as 64 billion edges. The underlying algorithm and ideas generalize from finding and monitoring subgraphs to the more general problem of computing and maintaining relational equi-joins over dynamic relations.

==> bigjoin-skew-resilient.tex <==
\section{BiGJoin-S: Handling Skew}
\label{sec:skew}
Although BiGJoin is worst-case optimal in terms of its cumulative computation and communication costs and requires small cumulative memory, it can generate imbalances in terms of how these costs are distributed across the machines in the cluster. There are two sources of skew in BiGJoin:
\begin{itemize}
\item {\em Size of indices:} Recall that in BiGJoin the $Ext^i_{a_{x_{ik}}}$ indices are distributed randomly yet for each prefix $p$, a single machine stores the entire extensions of $p$, i.e., the $S_p$ in the the prefix-extension pair $(p, S_p)$. In graph terms, this corresponds to a single machine storing all of the neighbors of a vertex. In skewed input data, this may generate imbalances in the amount of data indexed at each machine.
\item {\em Intersections and sizes of $P_k$'s:} BiGJoin starts a round of {\code Intersect Start} and {\code Intersect} phase when at least one machine has $B'$ amount of intersection work to do for the prefixes that it holds in $P_{k^*}$. However, the sizes of the $P_{k^*}$ prefixes in each machine might be skewed. It is likely for example that only one machine starts intersecting $B'$ extensions and other machines have no extensions to intersect. In addition there is no guarantee that during the {\code Intersection} stage each machine receives an equal number of intersection requests.

\end{itemize}

We next show a modification of BiGJoin, which we call BiGJoin-S, for {\em skew-resilient} that handles these sources of skew and maintains the cumulative computation, communication, and memory costs of BiGJoin and in addition ensures that each machine incurs asymptotically equal share of these costs. We start by describing the indices BiGJoin-S stores and then the stages of computation it executes. 

\subsection{Skew-resilient Indices}
BiGJoin-S stores three indices.
\begin{enumerate}
\item {\code Ext-Resolve} {\em Index:} For each prefix $p$ of each relation, instead of storing the prefix-extension pairs $(p, S_p)$ in a single machine, BiGJoin-S indices each extension of each prefix separately as follows. Suppose the $|S_p|$ extensions of $p$ are $e_1, e_2, ..., e_{|S_p|}$. We index $(p, 1)=e_1$, $(p, 2)=e_2$, ..., $(p, |S_p|)=e_{|S_p|}$. The {\code Ext-Resolve} index will be used to resolve the $j$th extension of each prefix through a distributed lookup. 

\item {\code Prefix-Exists} {\em Index: } Each prefix $p$ of each relation is randomly hashed to a machine. The {\code Prefix-Exists} index will be used during intersection to check if a resolved extension $(p \bullet e_j)$ exists in other relations.

\item {\code Count} {\em Index:} Fore each prefix $p$ of each relation, the tuple $(p, |S_p|)$ is hashed to a machine. The {\code Count} index will be used in the {\code Min-Count} stage to find the relation that contains the minimum number of extensions for $p$.
\end{enumerate}
We note two things. First, for each relation $R_i$ there will be $r_i$ {\code Ext-Resolve}, {\code Prefix-Exists}, and {\code Count} indices, one for each attribute that $R_i$ has. In the rest of our description of BiGJoin-S, when we say that we do a distributed lookup in any of these indices, the relation $R_i$ of the index will be clear from context.
Second, we note that since each $p$ and $(p, e_j)$ tuple is randomly hashed, under perfect hashing, each machine will receive equal amount of data to index w.h.p. Moreover, any distributed lookup on any index will be directed to each machine with $1/W$ probability.

\begin{figure}[t!]
  \centering
	\includegraphics[width=0.4\textwidth]{bigjoin-s-stages.jpg}
  \caption{Stages of BiGJoin-S.}
  \label{fig:bigjoin-s-stages}
\end{figure}


\subsection{Algorithm}
Figure~\ref{fig:bigjoin-s-stages} shows the stages of BiGJoin-S. Instead of BiGJoin's {\code Intersection-Start} stage, BiGJoin-S has a {\code Extension Resolving} stage. In addition, BiGJoin-S has one other {\code Balance} stage that ensures that the amount of $P_k$'s in each machine and the amount of intersection work done by each machine is balanced. There are two main differences between BiGJoin and BiGJoin-S: 

\begin{enumerate}
\item Similar to BiGJoin, for each machine $w_j$ holds a partition of $P_k$. Recall that in BiGJoin, for each prefix $p$ in $P_k$ one machine $w_j$ would store a ({\code p}, {\code min-r(p)}, {\code min-c(p)}, {\code offset(p)}) tuple. Instead in BiGJoin-S, one or more machines hold ({\code p},  {\code min-r(p)}, {\code start}, {\code end}) tuples, where the {\code start} and {\code end} indicate the range of indices within the $|S_p|$ extensions of $p$ that $w_j$ is responsible for extending. Therefore, {\code end} $-$ {\code start} gives the intersection work that machine $w_j$ has to do for $p$. BiGJoin-S's {\code Balance} stage ensures that the total intersection work that each machine has to do for the prefixes that it holds is balanced.

\item Instead of starting the cycle of stages from the $P_k$ with the largest $k$ value such that at least one machine has $B'$ intersection work to do, BiGJoin-S starts from the largest $k$ value such that all of the machines have at least $B'$ work to do. 

\end{enumerate}
We will again let $P_{k^*}$ be the prefix set that BiGJoin-S picks. We describe and analyze the costs of a cycle of BiGJoin-S's stages starting from {\code Extension Resolving} stage to the {\code Balance} stage. 

\noindent {\bf {\code Extension Resolving:}} Each machine $w_j$ takes exactly $B'$ intersection work from its ({\code p},  {\code min-r(p)}, {\code start}, {\code end}) tuples and first {\em resolves} each of the $(p, j)$ index in the [{\code start}, {\code end}] ranges of the picked tuples. This is done by doing a distributed lookup in the {\code Ext-Resolve} index of relation  {\code min-r(p)}.

\noindent {\bf {\code Intersect}:} Each machine, for each of the $B'$ prefixes that it resolved checks whether the resolved $(p \bullet e_j)$ prefix exists in each relation that contains attribute $a_{k^*+1}$. This is done by doing a distributed lookup in the relevant {\code Prefix-Exists} index of each relation that contains attribute $a_{k^*+1}$. If all of the indices contain $(p \bullet e_j)$, then $(p \bullet e_j)$ becomes a prefix in $P_{k^*+1}$. Otherwise it is discarded.

\noindent  {\bf {\code Min-Count}:} Each machine, for each successful $(p \bullet e_j)$ prefix in $P_{k^*+1}$ does a distributed lookup in the {\code Count} indices of all of the relations that contain attribute $a_{k^*+2}$ to find the {\code min-c($p \bullet e_j)$} and {\code min-r($p \bullet e_j$)} values of $(p \bullet e_j)$. This stage constructs {\code ($p \bullet e_j$},  {\code min-r($p \bullet e_j)$}, {\code start}=0, {\code end}={\code min-c($p \bullet e_j$)}) tuples.

\noindent  {\bf {\code Balance}:} Each {\code ($p \bullet e_j$,} {\code min-r($p \bullet e_j$)}, {\code min-c($p \bullet e_j)$}) tuples represents {\code min-c($p \bullet e_j$)} intersection work for the $p \bullet e_j$ prefix in $P_{k^* + 1}$. There may be an imbalance in how much intersection work each machine $w_j$ gets at this point. To balance this intersection work, each machine deterministically distributes its total intersection work generated in this cycle equally (with a +/- 1 difference) among the other machines. Each machine first finds the target intersection work amount $T$ to distribute to each machine. Then, each machine $w$  starts with an arbitrary other machine $w'$. Machine $w$ picks each tuple {\code $t=(p \bullet e_j$}, {\code min-r($p \bullet e_j$)}, {\code start}=0, {\code end}={\code min-c($p \bullet e_j)$}) and greedily gives as much of the work in $t$ to $w'$ (by picking an appropriate {\code start} and {\code end} range) until $w'$ gets exactly $T$ intersection work. Then $w$ moves to another machine and repeats the process. Note that this greedy procedure may split a tuple $t$ into multiple tuples, yet overall for each machine $w'$ we will generate at most $1$ new tuple (only for the last tuple that $w$ gives to $w'$). Therefore cumulatively, this process will generate at most $W$ new tuples for each machine $w$.

We next prove that BiGJoin-S balances all of the costs of BiGJoin equally across the $W$ machines and maintains BiGJoin's cumulative computation, communication, and memory costs.

\begin{theorem}
Suppose $B' \ge W$ and $B=WB' > \log(\IN \times MaxOut_Q)$. Then BiGJoin-S has the following costs:
\begin{itemize}
\item BiGJoin-S incurs a cumulative computation and communication cost of $O(mnMaxOut_Q)$ and cumulative memory cost of $O(mn\IN + mB)$.
\item BiGJoin-S requires $O(\frac{mnMaxOut_Q}{B})$ rounds of computation.
\item With at least  probability $1 - O(\frac{1}{\IN})$, each machine performs $\Theta(nB')$ communication and computation in every four stage cycles of BiGJoin. Moreover each machine, with at least $1-\frac{1}{e^{O(mn\IN)}}$ probability, requires at most  $O(\frac{mn\IN + mB}{W})$ memory.
\end{itemize}
\end{theorem}
\begin{proof}
First observe that similar to BiGJoin, for each prefix $p$, BiGJoin-S does $O(n)$ work in the {\code Min-Count} stage and  $O(n*\text{{\code min-c}}(p))$ computation and communication in the {\code Extension Resolving} and {\code Intersect} stages. Note also that the work done in {\code Balance} for $p$ is dominated by the work done in {\code Intersect} stage because for each worker that  $(p, {\text {\code min-r}(p)}, {\code start}, {\code end})$ tuples is sent to, there is at least one intersection that will be performed. This proves that the cumulative computation and communication costs of BiGJoin-S and BiGJoin are asymptotically the same.

Next, we prove that at any point in time the total number of $(p, {\text {\code min-r}(p)}, {\code start}, {\code end})$ tuples in $P_k$ never exceeds $4B$. This is an invariant of BiGJoin-S. Note that initially the invariant holds. Then suppose that at some point in time BiGJoin-S picks a $k^*$ to start extending $B$ tuples from. This implies that not every machine had at least $B'$ intersection work and therefore $B'$ many $P_{k^*+1}$ tuples. Since BiGJoin-S balances the amount of intersections that each machine has (with possibly a small +/- W imbalance), the total $P_{k^*+1}$ tuples were less than $W(B'+W)=B + W^2 \le 2B$. By extending $B$ many $P_{k^*}$ tuples, BiGJoin-S generates more $P_{k^*+1}$ tuples. However note that extending $B$ tuples cannot generate more than $2B$ tuples, completing the proof of the invariant. Therefore the total cumulative memory BiGJoin-S uses is $O(mn\IN + mB)$, where $O(mn\IN)$ is the memory cost of storing the indices and $mB$ is the cost of storing the $P_k$ prefix tuples. 

Next, note that similar to BiGJoin, each cycle of computation takes $O(mn)$ rounds. Since BiGJoin-S performs exactly $B$ intersections in each cycle, there are at most $O(\frac{MaxOut_Q}{B})$ cycles that BiGJoin-S performs, proving that BiGJoin-S takes $O(\frac{mnMaxOut_Q}{B})$ rounds in total.

We next analyze the per machine memory cost. First note that since we assume perfect hashing and each tuple in each index is stored independently in a random machine, by standard Chernoff bounds, the amount of data that each machine gets to index is  $O(\frac{mn\IN}{W})$ with probability at least $1-\frac{1}{e^{O(mnIN)}}$. Moreover since the amount of $P_k$ tuples stored is always balanced and we argued that the total $P_k$ tuples at any point do not exceed $4B$, the total per-machine memory does not exceed $O(\frac{mn\IN + mB}{W})$. 

Finally, we analyze the per-machine communication and computation costs in any cycle of BiGJoin-S. First note that in the {\code Extension-Resolving} stage, each machine does exactly $B'$ distributed lookups in {\code Ext-Resolve} indices. Note that since there are $B=B'W$ total lookups and we assume that $B > \log(\IN \times MaxOut_Q)$, by Chernoff bounds each machine receives $\Theta(B)$ lookup requests to its {\code Count} indices with probability at least $1 - \frac{1}{e^{\log(\IN \times MaxOut_Q)}} = 1-\frac{1}{\IN \times MaxOut_Q}$. Then similarly, in the {\code Intersect} stage, each machine does exactly $qB'$ lookups where $q \ge 1$ is the number of relations that contain attribute $a_{k^* + 1}$. By the same argument done for {\code Ext-Resolve} indices, each machine will therefore get $O(nB')$ (not $\Theta$) lookup requests. Finally at the end of the {\code Intersect} stage, each machine gets at most $B'$ new prefixes (if every single prefix they extended successfully intersected). In the {\code MinCount} stage each machine will do at most $nB'$ {\code Count} lookups and get $O(nB')$ work (instead of $\Theta(nB')$ with probability at least $1-\frac{1}{\IN \times MaxOut_Q}$. Finally in the {\code Balance} stage each worker will send and receive at most $O(B')$ tuples. Since each index lookup and the sending of a tuple in the {\code Balance} stage constitutes one unit of computation and communication, in each cycle, with probability at least $1-O(\frac{1}{\IN \times MaxOut_Q})$, each machine  does $\Theta(nB')$ work in any cycle. Since there are at most $MaxOut_Q$ cycles, with probability at least $1-O(\frac{1}{\IN})$, each machine incurs the same amount of communication and computation up to constants, completing the proof. 
\end{proof}

We note that we can make Delta-BiGJoin also skew-resilient under large enough updates by using BiGJoin-S with delta queries instead of BiGJoin. We need the update sizes, i.e., the size of the $Delta$-edges table, to be large enough to make Delta-BiGJoin-S skew-resilient. For example if each update to the relations contain a single tuple, then the amount of work to maintain the query results could be too small to possibly distribute equally across machines.

%Note that an immediate corollary to the theorem is that since there are at most $MaxOut_Q$ cycles, with probability at least $1-\frac{1}{\IN}$, each machine incurs the same amount of communication and computation up to constants. 
% within each cycle each machine will generate at most $W$ new tuples 
% constructs a subset of 
%($p \bullet e_j, {\code min-r(p \bullet e_j)}, {\code min-c(p \bullet e_j)})
%$({\code p \bullet e_j},  {\code min-r(p \bullet e_j)}, {\code start}, {\code end})$ offsets that add up to $T$, possibly not giving all of the ${\code min-c(p \bullet e_j$ work of the l
%($p \bullet e_j, {\code min-r(p \bullet e_j)}, {\code min-c(p \bullet e_j)}) and {\code 
%$ resolved, each machine 
%Let $INT_k$ be the total intersection work that needs to be done for all prefixes in $P_k$ at any point in time. BiGJoin-S maintains the invariant that the total intersection work that each machine $w_j$ has for the prefixes in each $P_k$ is equal to $\frac{INT_k}{W} +/- W$. 
%For each prefix $p$ in $P_k$, 
%  in $w_j$'s partition,  $w_j$ stores a tuple ({\code p}, {\code min-r(p)}, {\code min-c(p)}, \linebreak {\code offset(p)}). {\code min-r(p)} 
%This way of indexing, as well as other computations performed in BiGJoin, might cause workload imbalance across machines, which we will fix in Section~\ref{sec:skew}.
% As we discussed in Section~\ref{sec:big join}.
%Stages in BiGJoin-S:
%Prefix Resolving Stage: B' w.h.p.
%Intersection Stage: O(B') w.h.p.
%Balancing Stage For Extended Prefixes: < B' + W work so < 2B' work 
%Min-Count Stage: < B' work 
%Balancing Stage For Extensions: < B' work per machine
%
%So overall \Theta(B') work in each cycle. Therefore the total communication and computation work done by each machine is balanced. In addition observe that the cumulative communication and computation work done by BiGJoin-S is still O(mnMaxOut_Q). This is true because similar to BiGJoin, for each prefix p, BiGJoin-S also does O(n*min-c(p)) communication and computation as GJ does computation on p. For Min-Count stage, it performs O(n) work to discover the min-c(p) value and the relation. For each min-c(p) extensions of p, it does at most 2 communication when balancing the extensions of p. BiGJoin-S does O(min-c(p)) work when resolving the min-c(p) extensions of p. BiGJoin-S performs O(n) communication and computation cost when intersecting each min-c(p) extension of p. Finally it performs O(min-c(p)) communication and computation when balancing the at most O(min-c(p)) successfully extended subset of the possible min-c(p) extensions. Therefore, the total amount of work is O(mnMaxOut_Q). Since w.h.p. in each cycles of the 5 stages each machine does \Theta(B') work, w.h.p each machine does \Theta(mnMaxOut_Q/W) work.


==> deltabigjoin.tex <==
\section{Delta-BiGJoin}
\label{sec:delta-bigjoin}
We next describe the Delta-BiGJoin algorithm for evaluating continuous subgraph queries. Observe that since a given subgraph query $Q$ can be expressed as multiway joins of the {\code edges} table of an input graph $G$, we can use incremental view maintenance (IVM)  techniques for {\em join views}, i.e., views corresponding to joins of multiple tables, to continuously detect changes to the output of $Q$. Doing so would detect the emerged and deleted subgraphs that match $Q$ in $G$. Delta-BiGJoin is based on the IVM techniques from references~\cite{blakeley:ivm, gupta:ivm} which derive a set of delta queries $dQ1, ..., dQn$ (originally referred to as {\em delta rules}~\cite{gupta:ivm}) for $Q$ and evaluate each $dQi$ as the input tables change to maintain the result of $Q$.
We note that although the idea of delta queries is not new, our evaluation of $dQi$ using a worst-case join algorithm has theoretical implications that do not exist for existing incremental view maintenance algorithms that use delta queries, such as~\cite{blakeley:ivm, gupta:ivm}. Specifically, we show that under insertion-only workloads, if the delta queries are evaluated using the worst-case optimal GJ algorithm with specific attribute orderings, the total computation done to incrementally maintain the original join query is worst-case optimal up to constants that depend on on $Q$. 

We first review the technique of delta queries, and then describe our serial Delta-GJ algorithm, which evaluates these delta queries using the worst-case GJ algorithm. We then prove Delta-GJ's worst-case optimality in terms of computation cost under insertion-only workloads. In the distributed setting, the Delta-BiGJoin algorithm, which uses BiGJoin instead of GJ, gives us a worst-case optimal algorithm both in terms of computation and communication that also uses a small amount of cluster memory  under insertion-only workloads.


\subsection{Delta Join Queries}
Let $Q$ be a multiway join query as before and assume that one or more of the base tables are updated at a particular point in time. Let $\Delta R_i$, for each $i$, be a set of insertions or deleted tuples to relation $R_i$ in this update. We assume that tuples in each $\Delta R_i$ are labeled such that we can tell the inserted tuples apart from the deleted ones. Let $R_i'$ be $R_i \cup \Delta R_i$, where the union operation removes a tuple $t$ in $R_i$ if $\Delta R_i$ contains a deletion of $t$. Let $Out$ and $Out'$ be the output of $Q$ before and after the updates to the base relations, respectively. Then consider the following $n$ delta queries:
$$dQ_1 := \Delta R_1, R_2, R_3, ..., R_n$$
$$dQ_2 := R_1', \Delta R_2, R_3, ..., R_n$$ 
$$dQ_3 := R_1', R_2', \Delta R_3, R_4, ..., R_n$$ 
$$...$$
$$dQ_n := R_1', R_2', R_3', ..., \Delta R_n$$ 
When evaluating each $dQ_i$ if a deleted tuple from $\Delta R_i$ joins with tuples from the other $n-1$ relations and forms an output, $dR_i$ contains an output tuple that will be labeled as deleted. It can be shown~\cite{blakeley:ivm, gupta:ivm} that $Q' \setminus Q = dQ_1 \cup dQ_2 \cup ... \cup dQ_n$. That is evaluating the union of the $n$ queries above gives exactly the changes to the output of $Q$. We give an example.

\begin{example} 
Consider continuously evaluating the triangle query from Section~\ref{sec:preliminaries}. Suppose initially the graph is as in Figure~\ref{fig:ex-input-graph} with an extra edge (2, 8) (not shown in Figure~\ref{fig:ex-input-graph}). This graph already has two groups of three symmetric triangles (1, 6, 7), (6, 7, 1), (7, 1, 6) and (2, 6, 8), (6, 8, 2), (8, 2, 6).
Consider adding edges (10, 4), (11, 5) and deleting the edges (6, 11) and (7, 1) from this graph. Figure~\ref{fig:ex-input-graph-delta-gj} shows the new graph that forms after this update. In the figure, old edges are drawn in black color, new edges are drawn in green color, and the deleted edges are drawn in red color with dashes. Note that in the new graph, there are again two groups of three symmetric triangles: (2, 6, 8), (6, 8, 2), (8, 2, 6), which already existed and (4, 6, 10), (6, 10, 4), (10, 4, 6), which emerged after the update. In Figure~\ref{fig:ex-input-graph-delta-gj}, the edges of the emerged triangles are drawn thicker. Therefore we expect to detect as part of the update three deleted triangles (1, 6, 7), (6, 7, 1), (7, 1, 6) and three newly emerged triangles (4, 6, 10), (6, 10, 4), (10, 4, 6). 

Figure~\ref{fig:ex-input-edges-table-delta-gj} shows the {\code edges}, {\code $\Delta$edges}, and {\code edges'} tables. Now consider executing the three delta queries that would correspond to the triangle query. Since each table in our example has the same name, we name the delta queries as $dQ1$, $dQ2$, and $dQ3$.
\begin{itemize}
\item $dQ1(a_1, a_2, a_3) :- \Delta edges(a_1, a_2), edges(a_2, a_3), edges(a_3, a_1)$: The output of $dQ1$ is \{(7, 1, 6)-,
(10, 4, 6)+, (11, 5, 6)+\}, where +/- indicate whether the output tuple is inserted or deleted, corresponding to whether the triangle has emerged or has been deleted. Notice that (11, 5, 6) is actually not a triangle that actually has emerged. As we will see $dQ3$ will have the (11, 5, 6)- output, so when we union the outputs, we will not get the (11, 5, 6) tuple in the final changes to the output.
\item $dQ2(a_1, a_2, a_3) :- edges'(a_1, a_2), \Delta edges(a_2, a_3), edges(a_3, a_1)$: The output of $dQ2$ is \{(6, 7, 1)-, (6, 10, 4)+\}.
\item $dQ3(a_1, a_2, a_3) :- edges'(a_1, a_2), edges'(a_2, a_3), \Delta edges(a_3, a_1)$: The output of $dQ2$ is \{(1, 6, 7)-, (4, 6, 10)+, (11, 5,  6)-\}.
\end{itemize}
As we see, the union of the outputs of $dQ1$, $dQ2$, and $dQ3$ gives us exactly \{ (1, 6, 7)-, (6, 7, 1)-, (7, 1, 6)-, (4, 6, 10)+, (6, 10, 4)+, (10, 4, 6)+\}.
\end{example}

\begin{figure}[t!]
  \centering
	\includegraphics[width=0.25\textwidth]{ex-input-graph-delta-gj.jpg}
  \caption{Input graph to Delta-GJ.}
  \label{fig:ex-input-graph-delta-gj}
  \vspace{-10pt}
\end{figure}

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{.32\textwidth}
  \centering
\includegraphics[height=0.31\textwidth]{ex-delta-edges-table-delta-gj.jpg}
  \caption{{\code $\Delta$edges} table}
  \label{fig:ex-edge-tables-delta-gj}
\end{subfigure}
\begin{subfigure}[b]{.32\textwidth}
  \centering
\includegraphics[height=0.8\textwidth]{ex-edge-table-delta-gj.jpg}
  \caption{{\code edges} table.}
  \label{fig:ex-edge-tables-delta-gj}
\end{subfigure}
\begin{subfigure}[b]{.32\textwidth}
  \centering
\includegraphics[height=0.8\textwidth]{ex-edges-prime-table-delta-gj.jpg}
  \caption{{\code edges'} table.}
  \label{fig:ex-edge-tables-delta-gj}
\end{subfigure}
\caption{Example input graph and its edge table.}
\label{fig:ex-input-edges-table-delta-gj}
\vspace{-10pt}
\end{figure*}

\subsection{Delta-GJ and Delta-BiGJoin}
Delta-GJ runs  the $n$ delta queries of $Q$ one after another in the order of $dQ_1, ..., dQ_n$ using GJ. Note that Delta-GJ's correctness, i.e., that it finds the correct differences to the output of $Q$, simply follows from the correctness of the delta query technique~\cite{blakeley:ivm, gupta:ivm}. Note also that Delta-GJ's correctness does not depend on the attribute ordering that it picks. However, in order to prove that Delta-GJ executes each delta query $dR_i$ efficiently, we will need to do two things:
\begin{itemize}
\item{\bf Attribute ordering}: For $dR_i$, Delta-GJ picks an attribute ordering that starts with any permutation of $R_i$'s attributes $a_{i1}, a_{i2}, ..., a_{ir_i}$ and an arbitrary order for the remaining $m - r_i$ attributes. For example if $R_3(a_2, a_4)$ is a relation in $Q$ and there are 4 attributes $a_1$, $a_2$, $a_3$, and $a_4$ in $Q$, then for $dQ_3$ Delta-GJ can pick one of the following attribute orderings: $<$$a_2, a_4, a_1, a_3$$>$, $<$$a_2, a_4, a_3, a_1$$>$, $<$$a_4, a_2, a_1, a_3$$>$, and  $<$$a_4, a_2, a_3, a_1$$>$.

\item{\bf Indexing of tuples in $\Delta R_i$ and omitting the computation of $P_1$, ..., $P_{r_i-1}$}: In order to run GJ on $dQ_i$, Delta-GJ needs to construct extension indices for $\Delta R_i$. We refer to these indices as $\Delta{\text -}Ext^i_{a_{x_{ik}}}$ to distinguish them from $Ext^i_{a_{x_{ik}}}$ indices that index $R_i$. $\Delta{\text -}Ext^i_{a_{x_{ik}}}$ are only used for evaluating $dR_i$. After $dR_i$ is evaluated, Delta-GJ deletes $\Delta{\text -}Ext^i_{a_{x_{ik}}}$ indices and integrates $\Delta R_i$ into $Ext^i_{a_{x_{ik}}}$, which now reflects the state of $R_i$ after applying $\Delta R_i$. After indexing each tuple $t=(a_{i1}^*, a_{i2}^*, ..., a_{ir_i}^*)$ in $\Delta R_i$ into $\Delta{\text -}Delta-GJ_{a_{x_{ik}}}$, Delta-GJ then checks if $t$ is a possible $P_{r_i}$ tuple. Assume w.l.o.g. that Delta-GJ has picked $a_{i1}, a_{i2}, ..., a_{ir_i}$ as the first $r_i$ set of attributes in the global ordering of attributes in $dR_i$. We simply check in each $Ext^j_{a_{i1}}$ whether $a_{i1}^*$ exists. If so, we then check if $Ext^j_{a_{i2}}[(a_{i1}^*)]$ contains $a_{i2}^*$. Note that each of these lookups is a constant operation because we are checking only one element in each lookup. Therefore in $O(mn)$ time we can check if $t$ is in $P_{r_i}$ or not. Delta-GJ computes $P_{r_i}$ this way and avoids an explicit computation of  $P_1$, ..., $P_{r_i-1}$. Computation of $P_{r_i + 1}$ to $P_{m}$ is done as before.
\end{itemize}

We next argue that under insertion-only workloads, Delta-GJ's cumulative computation cost at any point in time is worst-case optimal (up to constants that depend on the query), in a sense that we make formal in the following theorem. Before we state the theorem we need to introduce some notation. Consider a query $Q$ and consider a series of updates, $\Delta(1), \Delta(2), ...$, that modify the input relations $R_i$ of $Q$. We denote by $\Delta R_i(z)$ the set of updates to $R_i$ in $\Delta(z)$. We denote by $R_i(z)$ the state of relation $R_i$ after incorporating all of the updates until and including $\Delta R_i (z)$, i.e., $R_i(z) = \Delta R_i(1) \cup \Delta R_i(2) \cup ... \cup \Delta R_i(z)$.

\begin{theorem}
\label{thm:delta-gj}
Consider a query $Q$ and a series of $z$ updates that only consist of inserting tuples to the input relations of $Q$. Then the total computation cost of Delta-GJ is $O(mn^2MaxOut_Q)$, where $MaxOut_Q$ is the AGM bound of $Q$ on $R_i(z)$.
\end{theorem}

\begin{proof}
Delta-GJ evaluates each $dQ_i$ $z$ times, one for each update. For each $dQ_i$ we show that the cumulative cost of these $z$ evaluations is less than running $GJ$ on $R_i(z)$ with the same attribute ordering Delta-GJ uses for $dQ_i$. We let the query that GJ evaluates on the final relations as $Q(z) := R_1(z), ..., R_n(z)$. Note that by Theorem~\ref{thm:gj}, the cost of running GJ with any attribute ordering is $O(mnMaxOut_Q)$. The claim of the theorem then follows from the fact that there are $n$ delta queries. We need to account for Delta-GJ's three costs when evaluating $dQ_i$ $z$ times: (1) Cost of indexing; (2) Cost of computing $P_{r_i}$ tuples; and (3) Cost of computing the rest of $P_{r_i + 1}, ..., P_{m}$. 

For cost (1), note that the cost of indexing each tuple $t$ in $\Delta R_i(1), ..., \Delta R_i(z)$ first into $r_i$ $\Delta{\text -}Ext^i_{a_{x_{ik}}}$ and then into  $r_i$ $Ext^i_{a_{x_{ik}}}$ indices does not asymptotically change the indexing cost of running $GJ$ when evaluating $Q$ on $R_i(z)$ (it only doubles the cost).

For cost (3), note that once $P_{r_i}$ have been computed, the cost of Delta-GJ for extending any tuple $t \in P_{r_i}$ to $P_j$ for $r_i < j \le m$ is clearly less than the cost that GJ incurs when extending $t$ when GJ fixes the same global attribute ordering as Delta-GJ. This is because by definition, $dQ_i := R_1(z), R_2(z), ..., dR_i, R_i(z-1), ..., R_n(z-1)$ and each relation in $dQ_i$ is a subset of its corresponding relation in $Q(z)$

Finally for cost (2). Recall that Delta-GJ incurs a cost of $O(mn)$ for each tuple $t \in \Delta R_i$  to verify whether $t$ is in $P_{r_i}$ or not. Cumulatively across all of the $z$ updates, these checks incur an extra cost of $O(mn|R_i(z)|)$. Moreover, cumulatively across all of the $dR_i$, this cost is  $O(mn\IN)$. We note that in the best case $MaxOut_Q$ is $\Omega(\frac{\IN}{n})$, since the largest relation is of size at least $\frac{\IN}{n}$ and the worst-case output of any query is at least the size of its largest relation. Therefore $mn^2MaxOut_Q$ is at least $mn\IN$, which implies that  $O(mn\IN)$ is a cost that is subsumed by $O(mn^2MaxOut_Q)$, completing the proof.
\end{proof}
We note that it is plausible to analyze Delta-GJ's optimality under workloads including deletions using other notions of optimality, such as the {\em trace edit distance} used in reference~\cite{veldhuizen:inc-lftj}. We leave this to future work. 
%We note that the meaning of worst-case optimality is not well defined when we consider deletions, as the size of the tables might decrease, resulting in the value of  $MaxOut_Q$ to decrease from update to update despite forcing any algorithm to do more computation. However, it is plausible to analyze algorithms' optimality under general workloads using other notions of optimality, such as the {\em trace edit distance} used in reference~\cite{veldhuizen:inc-lftj} for incremental view maintenance algorithms. We leave this to future work. 


% DO NOT REMOVE. REUSABLE BLURB
% We note that the meaning of worst-case optimality is not well defined when we consider deletions. That is because, suppose in the first update we insert a large number of tuples to each relation $R_i$. Then in the second updates we remove all of these tuples. Then since the input relations will be empty, $MaxOut_Q$ after update $2$ will be 0, yet clearly any IVM algorithm needs to detect the emergence and deletions of all of the tuples at the end of the first update. Therefore, we ignore the analysis of Delta-GJ under general workloads that consist of both insertions and deletions. However, it is plausible to analyze algorithms' optimality under general workloads using other notions of optimality. We leave this to future work. 

Our Delta-BiGJoin algorithm simply runs BiGJoin on each delta query in the distributed setting. For each tuple $t$, in parallel, in $\Delta R_i$, we also replace the lookups in the extension indices to verify whether $t$ is in $P_{r_i}$ by distributed lookups, incurring at most $O(mn)$ communication, computation, and rounds. We next state a theorem about Delta-BiGJoin's costs.


\begin{theorem}
\label{thm:delta-bigjoin}
Consider a query $Q$ and a series of $z$ insertion-only updates to the input relations of $Q$. Let $\IN(z)$ denote $\sum_i |R_i(z)|$. Then, given a batch size $B'$, Delta-BiGJoin's communication and computation cost under insertion-only workloads is $O(mn^2MaxOut_Q)$. The cumulative memory Delta-BiGJoin takes is $O(mn\IN(z) + mWB')$. The number of rounds of computation Delta-BiGJoin takes is $O(mn^2\frac{MaxOut_Q}{B'} + zmn^2)$.
\end{theorem}

\begin{proof}
Note that by Thereom~\ref{thm:gj} BiGJoin's communication and computation cost on any query $Q$ is asymptotically same as the computation cost of running GJ on $Q$. By the same arguments in Theorem~\ref{thm:delta-gj}, the communication and computation cost of Delta-BiGJoin is therefore  $O(mn^2MaxOut_Q)$. Note also that the cumulative memory cost of Delta-BiGJoin is never larger than the  $O(mn\IN(z) + mWB')$ memory cost of running GJ on $Q(z)$. This is because at any point in time, the indices that Delta-BiGJoin uses is at most as large as the indices that GJ uses on $Q(z)$. Similarly, the intermediate data that Delta-BiGJoin generates on any $dQ_i$ query is at most as large the intermediate data that GJ generates on $Q(z)$.  For the number of rounds, note that after each update, Delta-BiGJoin runs $O(mn)$ rounds of computation to compute $P_{r_i}$. From then on, the algorithm will extend prefixes and perform intersections using the same batch size of $B'$ as GJ does. Except, we note that for each update Delta-BiGJoin might run at most another extra $O(mn)$ rounds of computation if the updates are small or if they do not generate enough $P_{r_i +1}, ..., P_m$ prefixes. Note that cumulatively, Delta-GJ, for each $dQ_i$, computes the same $P_{r_i}$ as GJ does on $Q(z)$. Therefore, for each $dQ_i$, cumulatively across all of the $z$ updates, Delta-BiGJoin runs the same number of rounds as GJ does and an additional $O(zmn)$ rounds. Since there are $n$ delta queries, the total number of rounds of computation is  $O(mn^2\frac{MaxOut_Q}{B'} + zmn^2)$, completing the proof.
\end{proof}
